Back to the Basics: Revisiting Out-of-Distribution Detection Baselines

We study simple methods for out-of-distribution (OOD) image detection that are compatible with any already trained classifier, relying on only its predictions or learned representations. Evaluating the OOD detection performance of various methods when utilized with ResNet-50 and Swin Transformer models, we find methods that solely consider the model's predictions can be easily outperformed by also considering the learned representations. Based on our analysis, we advocate for a dead-simple approach that has been neglected in other studies: simply flag as OOD images whose average distance to their K nearest neighbors is large (in the representation space of an image classifier trained on the in-distribution data).

==> tables/test_tinytable.tex <==
\begin{table}[h!]
\vspace*{-2mm}
{\tiny 
\begin{center}
\caption{Lift at \# errors with Swin Transformer model.}

\begin{tabular}{lrrrrr}
\toprule
             Label Quality Score &  roman- &  food- &  cifar- &  cifar- &  cifar- \\
             & numeral & 101n & 10n-worst & 10n-agg & 10s 
             \\
\midrule
            Self Confidence &           4.05 &       3.80 &             2.36 &          10.34 &       4.94 \\
          Normalized Margin &           3.89 &       3.16 &             2.37 &          10.36 &       4.92 \\
   Adjusted Self Confidence &           4.11 &       3.42 &             2.35 &          10.35 &       4.87 \\
 Adjusted Normalized Margin &           3.85 &       3.33 &             2.38 &          10.37 &       4.92 \\
Confidence Weighted Entropy &           4.17 &       3.84 &             2.33 &          10.29 &       4.93 \\
                    Entropy &           3.01 &       2.81 &             1.28 &           3.59 &       0.52 \\
           Least Confidence &           2.84 &       2.73 &             1.32 &           3.67 &       0.61 \\
\bottomrule
\end{tabular}

\end{center}
}
\vspace*{-2mm}
\end{table}
